Native Chinese Reader: A Dataset Towards Native-Level Chinese Machine Reading Comprehension

We present Native Chinese Reader (NCR), a new machine reading comprehension (MRC) dataset with particularly long articles in both modern and classical Chinese. NCR is collected from the exam questions for the Chinese course in China's high schools, which are designed to evaluate the language proficiency of native Chinese youth. Existing Chinese MRC datasets are either domain-specific or focusing on short contexts of a few hundreds of characters in modern Chinese only. By contrast, NCR contains 8390 documents with an average length of 1024 characters covering a wide range of Chinese writing styles, including modern articles, classical literature and classical poetry. A total of 20477 questions on these documents also require strong reasoning abilities and common sense to figure out the correct answers. We implemented multiple baseline models using popular Chinese pre-trained models and additionally launched an online competition using our dataset to examine the limit of current methods. The best model achieves 59% test accuracy while human evaluation shows an average accuracy of 79%, which indicates a significant performance gap between current MRC models and native Chinese speakers. We release the dataset at https://sites.google.com/view/native-chinese-reader/.

==> 23_others.tex <==
\xss{
In addition to Chinese and English, there are also many MRC datasets in other languages such as Japanese\cite{shibuki2014overview, takahashi-etal-2019-machine}, Russian\cite{efimov2020sberquad} etc. along with some cross-lingual datasets\cite{artetxe2019cross, liu2019xqa}.
}

==> 24_model.tex <==

Ever since the release of BERT \cite{BERT}, pre-trained language model has become the main stream paradigm for NLP practitioners. As an increasing amount of corpus was crawled, the model also become larger and larger. Specifically, GPT-3 \cite{GPT3}, with more than 170 billion parameters, achieves amazing results in many downstream tasks even in few-shot setting, proving that models can really understand human language. However, the biggest problem of GPT-3 is that it lacks common sense and does not have cognitive abilities. GPT-3 still has a big gap with human intelligence in complex cognitive reasoning tasks, such as open domain dialogue, knowledge-based question answering, and controllable text generation, etc. In Chinese language, pre-trained models is also advancing fast and create new state of the art. Among them, M6 \cite{M6} and GLM \cite{GLM} are in the forefront. Our dataset is to test model's comprehension ability with common sense, so it would be a good benchmark for Chinese pre-trained model research.
Machine Reading Comprehension originated from the MCTest data set released by \newcite{MCTest}. in 2013. The format of MCTest is very similar to the single-choice question format of the English standardized test. It provides text, questions, and 4 options, and the model needs to determine the correct option. Answering the questions of the dataset does not require external knowledge, and the answers can be found from the text, which can be a good measure of the model's ability to understand language. Due to the small number of samples of MCTest (500 texts and 1,000 questions), it cannot be effectively trained in today's deep learning world driven by massive data. 

==> 33_table_modern.tex <==

\begin{table*}[]
    \footnotesize
    \centering
        \begin{tabular}{m{6cm} m{8.5cm}}
        \hline
        \begin{CJK}{UTF8}{gbsn}
        在酒楼上（节选）鲁迅
        % （1）楼上空空如也，任我拣得最好的坐位：可以眺望楼下的废园。这园大概是不属于酒家的，我先前也曾眺望过许多回，有时也在雪天里。但现在从惯于北方的眼睛看来，却很值得惊异了：几株老梅竟斗雪开着满树的繁花，仿佛毫不以深冬为意；倒塌的亭子边还有一株山茶树，从暗绿的密叶里显出十几朵红花来，赫赫的在雪中明得如火，愤怒而且傲慢，如蔑视游人的甘心于远行。
        ...（2）我竟不料在这里意外的遇见朋友了，——假如他现在还许我称他为朋友。那上来的分明是我的旧同窗，也是做教员时代的旧同事，面貌虽然颇有些改变，但一见也就认识，独有行动却变得格外迂缓，很不像当年敏捷精悍的吕纬甫了。
        % （3）我就邀他同坐，但他似乎略略踌躇之后，方才坐下来。我起先很以为奇，接着便有些悲伤，而且不快了。细看他相貌，也还是乱蓬蓬的须发；苍白的长方脸，然而衰瘦了。精神很沉静，或者却是颓唐；又浓又黑的眉毛底下的眼睛也失了精采，但当他缓缓的四顾的时候，却对废园忽地闪出我在学校时代常常看见的射人的光来。
        % （4）“我们，”我高兴的，然而颇不自然的说，“我们这一别，怕有十年了罢。我早知道你在济南，可是实在懒得太难，终于没有写一封信。……”（5）“彼此都一样。可是现在我在太原了，已经两年多，和我的母亲。我回来接她的时候，知道你早搬走了，搬得很干净。”（6）“你在太原做什么呢？”我问。（7）“教书，在一个同乡的家里。”（8）“这以前呢？”（9）“这以前么？”他从衣袋里掏出一支烟卷来，点了火衔在嘴里，看着喷出的烟雾，沉思似的说：“无非做了些无聊的事情，等于什么也没有做。”（10）他也问我别后的景况；我一面告诉他一个大概，一面叫堂倌先取杯筷来，使他先喝着我的酒，然后再去添二斤。其间还点菜，我们先前原是毫不客气的，但此刻却推让起来了。终于说不清那一样是谁点的，就从堂倌的口头报告上指定了四样莱：茴香豆，冻肉，油豆腐，青鱼干。
        （11）“我一回来，就想到我可笑。”他一手擎着烟卷，一只手扶着酒杯，似笑非笑的向我说。“我在少年时，看见蜂子或蝇子停在一个地方，给什么来一吓，即刻飞去了，但是飞了一个小圈子，便又回来停在原地点，便以为这实在很可笑，也可怜。可不料现在我自己也飞回来了，不过绕了点小圈子。又不料你也回来了。你不能飞得更远些么？”
        % （12）“这难说，大约也不外乎绕点小圈子罢。”我也似笑非笑的说。“但是你为什么飞回来的呢？”（13）“也还是为了无聊的事。”他一口喝干了一杯酒，吸几口烟，眼睛略为张大了。“无聊的。——但是我们就谈谈罢。”（14）堂倌搬上新添的酒菜来，排满了一桌，楼上又添了烟气和油豆腐的热气，仿佛热闹起来了；楼外的雪也越加纷纷的下。（15）“你也许本来知道，”他接着说，“我曾经有一个兄弟，是三岁上死掉的，就葬在这乡下。我连他的模样都记不清楚了，但母亲一知道就很着急，几乎几夜睡不着，——她又能自己看信的，然而我能有什么法子呢？没有钱，没有工夫：当时什么法也没有。一直挨到现在。待到掘着圹穴，我便过去看，果然，棺木已经快要烂尽了，只剩下一堆木丝和小木片。我的心颤动着，自去拨开这些，很小心的，要看一看我的小兄弟。”（16）我忽而看见他眼圈红了，但立即知道有了酒意。我叫堂倌再添二斤酒，然后回转身也拿着酒杯，正对面默默的听着。（17）“其实，这本已可以不必再迁，只要平了土，卖掉棺材，就此完事了的。但我不这样，我仍然铺好被褥，用棉花裹了些他先前身体所在地方的泥土，包起来，装在新棺材里，运到我父亲埋着的坟地上，在他坟旁埋掉了。这样总算完成了一件事，足够去骗骗我的母亲，使她安心些。——阿阿，你这样的看我，你怪我何以和先前太不相同了么？是的，也还记得我们同到城隍庙里去拔掉神像的胡子的时候，连日议论些改革中国的方法以至于打起来的时候。但我现在就是这样了。”（18）他又掏出一支烟卷来，衔在嘴里，点了火。
        （19）“……这些无聊的事算什么，只要模模胡胡。模模胡胡的过了新年，仍旧教我的‘子曰诗云’去。” （20）“你教的是‘子曰诗云’”么？我觉得奇异，便问。 （21）“自然。你还以为教的是ABCD么？我先是两个学生，一个读《诗经》，一个读《孟子》。新近又添了一个，女的，读《女儿经》。连算学也不教，不是我不教，他们不要教。” （22）“我实在料不到你倒去教这类书,...” （23）“他们的老子要他们读这些；我是别人，无乎不可的。这些无聊的事算什么？只要随随便便,...” （24）“那么，你以后豫备怎么办呢？” （25）“以后？——我不知道。你看我们那时豫想的事可有一件如意？我现在什么也不知道，连明天怎样也不知道，连后一分……” （26）堂倌送上账来，交给我；他也不像初时候的谦虚了，指向我看一眼，便吸烟听凭我付了账。
        % （27）我们一同走出店门，他所住的旅馆和我的方向正相反，就在门口分别了。我独自向着自己的旅馆走，寒风和雪片扑在脸上，倒觉得很爽快。见天色已是黄昏，和屋宇和街道都织在密雪的纯白而不定的罗网里。1924年2月16日
        \end{CJK} &
In the Wine Shop (Excerpt) Lu Xun 
(2) I never guessed that here of all places I should
expectedly meet a friend -- if such he would still let me call him. The newcomer was an old class mate who had been my colleague when I was a teacher, and although he had changed a great deal I knew him as soon as saw him. Only he had become much slower in his movements, very unlike the nimble and active Lu Wei-fu of the old days.
(11)``As soon as I came back I knew I was a fool''. Holding
his cigarette in one hand and the wine cup in the other, he
spoke with a bitter smile. `` When I was young, I saw the way
bees or flies stopped in one place. If they were frightened
they would fly but after flying in a small circle they would
come back again to stop in the same place; and I thought this really very foolish, as well as pathetic. But I didn't think that I would fly back myself, after only flying in a small circle.
And I didn't think you would come back either. Couldn't you
have flown a little further?''     
(19)``...Who cares about such futile affairs anyway? One only
wants to muddle through them somehow. When I have muddled through New Year I shall go back to teaching the Confucian classics as before.''
(20)``Are you teaching that?'' I asked in astonishment
(21)``Of course. Did you think I was teaching English? First
I had two pupils, one studying the Book of Songs, the other
Mencius. Recently I have got another, a girl, who is studying
the Canon for Girls. I don't even teach mathematics; not that
I wouldn't teach it, but they don't want it taught.''
(22)``I could really never have guessed that you would be teaching such books''
(23) ``Their father wants them to study these. I'm an outsider
so it's all the same to me. Who cares about such futile affairs
anyway There's no need to take them seriously ...''
(24) ``Then what do you mean to do in future?''
(25) ``In future? I don' t know. Just think: Has any single thing
turned out as we hoped of all we planned in the past? I'm not sure of anything now, not even of what I will do tomorrow, or even of the next minute ...''
(26) The waiter brought up the bill and gave it to me. Wei-fu
did not behave so formally as before, just glanced at me,
then went on smoking and allowed me to pay.
        \\
         \hline
        Q1 \begin{CJK}{UTF8}{gbsn}
        下列对文章思想内容的理解与分析，不正确的一项是
        \end{CJK}
         &
        Q1 The incorrect one from the following understanding and analysis of the thought content of the article is:\\
        A. \begin{CJK}{UTF8}{gbsn}
        “行动却变得格外迂缓，很不像当年敏捷精悍的吕纬甫了”高度概括了眼前吕纬甫的精神状态，突出他的迂缓颓废。
        \end{CJK} &
        A. `` Only he had becomemuch slower in his movements, very unlike the nimble and active LuWei-fu of the old days. '' gives a high-level overview of Lu Weifu's mental state, highlighting his sluggish decadence.\\
        B. \begin{CJK}{UTF8}{gbsn}
        “蝇子飞了一个小圈子，便又回来停在原地点”，吕纬甫的这番自述自嘲中对自身缺乏清醒的认识，浑噩度日，揭示了残酷的现实生活将人的灵魂挤扁，只能在颓唐消沉中磨蚀生命的主题。$\star$ 
        \end{CJK} & 
        B. ``If they were frightened they would fly but after flying in a small circle they would come backagain to stop in the same place.'' indicates that Lu Wei-fu lacks a clear understanding of himself and live in a muddle, which reveals that the cruel reality of life squeezes the human soul, and can only erode the life in depression and depression. \\
        C. \begin{CJK}{UTF8}{gbsn}
        从吕纬甫叙述现在教书生涯的内容和原因的话语中，可见他已经违背了当初的理想，变得苟且偷安，屈从于当前顽固封建势力。
        \end{CJK} & 
        C. From Lu Wei-fu's narration of the content and reasons of his current teaching career, it can be seen that he has violated his original ideals, has become stubborn, and yielded to the current stubborn feudal forces.\\
        D. \begin{CJK}{UTF8}{gbsn}
        文章通过吕纬甫的人生经历来告诉读者，吕纬甫的人生悲剧正是那个时代无数知识分子悲剧命运的代表，而个人的悲剧背后则是整个时代的悲哀。 
        \end{CJK} & 
        D. The article tells readers through Lu Wei-fu's life experience that Lu Weifu's life tragedy is the representative of the tragedy of countless intellectuals in that era, and behind the personal tragedy is the tragedy of the entire era.\\
        \\
        % Q2 \begin{CJK}{UTF8}{gbsn}
        % 下列对文章艺术特点的理解与鉴赏，不正确的一项是
        % \end{CJK}
        %  & \\
        % A. \begin{CJK}{UTF8}{gbsn}
        % 小说情节围绕吕纬甫的自述展开，他的叙述中有乡情，有友情，还有“迁坟”这件小事中流露出的人情 $\star$
        % \end{CJK} & \\
        % B. \begin{CJK}{UTF8}{gbsn}
        % 梅花、山茶与白雪共同构成了一幅充满生机与活力的画面，表现了鲁迅先生悲观中奋起、绝望中反抗的战斗精神。
        % \end{CJK} & \\
        % C. \begin{CJK}{UTF8}{gbsn}
        % 小说人物刻画体现出鲁迅先生简练传神的特色，极具个性化的人物语言，偶一闪现的肖像描写，颇耐人寻味。其中一句“也还是乱蓬蓬的须发”可让人生发许多联想。
        % \end{CJK} & \\
        % D. \begin{CJK}{UTF8}{gbsn}
        % 小说结尾含蓄深刻，意蕴无穷。“见天色已是黄昏，和屋宇和街道都织在密雪的纯白而不定的罗网里。” “罗网”是指封建文化思想依旧弥漫的社会环境。
        % \end{CJK} & \\
        % \\
    \hline
    \end{tabular}
    \caption{An example of document in Modern Chinese with question (left) and English translation (right), $\star$ is the correct option. To save space, we extract the sentences which is related to the question from the raw document.}
    \label{tab:modern_chinese}
\end{table*}


==> 34_table_modern_bak.tex <==
\begin{table*}[]
    \footnotesize
    \centering
        \begin{tabular}{m{16cm} m{0cm}}
        \hline
        \begin{CJK}{UTF8}{gbsn}
        在酒楼上（节选）鲁迅（1）楼上空空如也，任我拣得最好的坐位：可以眺望楼下的废园。这园大概是不属于酒家的，我先前也曾眺望过许多回，有时也在雪天里。但现在从惯于北方的眼睛看来，却很值得惊异了：几株老梅竟斗雪开着满树的繁花，仿佛毫不以深冬为意；倒塌的亭子边还有一株山茶树，从暗绿的密叶里显出十几朵红花来，赫赫的在雪中明得如火，愤怒而且傲慢，如蔑视游人的甘心于远行。（2）我竟不料在这里意外的遇见朋友了，——假如他现在还许我称他为朋友。那上来的分明是我的旧同窗，也是做教员时代的旧同事，面貌虽然颇有些改变，但一见也就认识，独有行动却变得格外迂缓，很不像当年敏捷精悍的吕纬甫了。 （3）我就邀他同坐，但他似乎略略踌躇之后，方才坐下来。我起先很以为奇，接着便有些悲伤，而且不快了。细看他相貌，也还是乱蓬蓬的须发；苍白的长方脸，然而衰瘦了。精神很沉静，或者却是颓唐；又浓又黑的眉毛底下的眼睛也失了精采，但当他缓缓的四顾的时候，却对废园忽地闪出我在学校时代常常看见的射人的光来。（4）“我们，”我高兴的，然而颇不自然的说，“我们这一别，怕有十年了罢。我早知道你在济南，可是实在懒得太难，终于没有写一封信。……”（5）“彼此都一样。可是现在我在太原了，已经两年多，和我的母亲。我回来接她的时候，知道你早搬走了，搬得很干净。”（6）“你在太原做什么呢？”我问。（7）“教书，在一个同乡的家里。”（8）“这以前呢？”（9）“这以前么？”他从衣袋里掏出一支烟卷来，点了火衔在嘴里，看着喷出的烟雾，沉思似的说：“无非做了些无聊的事情，等于什么也没有做。”（10）他也问我别后的景况；我一面告诉他一个大概，一面叫堂倌先取杯筷来，使他先喝着我的酒，然后再去添二斤。其间还点菜，我们先前原是毫不客气的，但此刻却推让起来了。终于说不清那一样是谁点的，就从堂倌的口头报告上指定了四样莱：茴香豆，冻肉，油豆腐，青鱼干。（11）“我一回来，就想到我可笑。”他一手擎着烟卷，一只手扶着酒杯，似笑非笑的向我说。“我在少年时，看见蜂子或蝇子停在一个地方，给什么来一吓，即刻飞去了，但是飞了一个小圈子，便又回来停在原地点，便以为这实在很可笑，也可怜。可不料现在我自己也飞回来了，不过绕了点小圈子。又不料你也回来了。你不能飞得更远些么？”（12）“这难说，大约也不外乎绕点小圈子罢。”我也似笑非笑的说。“但是你为什么飞回来的呢？”（13）“也还是为了无聊的事。”他一口喝干了一杯酒，吸几口烟，眼睛略为张大了。“无聊的。——但是我们就谈谈罢。”（14）堂倌搬上新添的酒菜来，排满了一桌，楼上又添了烟气和油豆腐的热气，仿佛热闹起来了；楼外的雪也越加纷纷的下。（15）“你也许本来知道，”他接着说，“我曾经有一个兄弟，是三岁上死掉的，就葬在这乡下。我连他的模样都记不清楚了，但母亲一知道就很着急，几乎几夜睡不着，——她又能自己看信的，然而我能有什么法子呢？没有钱，没有工夫：当时什么法也没有。一直挨到现在。待到掘着圹穴，我便过去看，果然，棺木已经快要烂尽了，只剩下一堆木丝和小木片。我的心颤动着，自去拨开这些，很小心的，要看一看我的小兄弟。”（16）我忽而看见他眼圈红了，但立即知道有了酒意。我叫堂倌再添二斤酒，然后回转身也拿着酒杯，正对面默默的听着。（17）“其实，这本已可以不必再迁，只要平了土，卖掉棺材，就此完事了的。但我不这样，我仍然铺好被褥，用棉花裹了些他先前身体所在地方的泥土，包起来，装在新棺材里，运到我父亲埋着的坟地上，在他坟旁埋掉了。这样总算完成了一件事，足够去骗骗我的母亲，使她安心些。——阿阿，你这样的看我，你怪我何以和先前太不相同了么？是的，也还记得我们同到城隍庙里去拔掉神像的胡子的时候，连日议论些改革中国的方法以至于打起来的时候。但我现在就是这样了。”（18）他又掏出一支烟卷来，衔在嘴里，点了火。（19）“……这些无聊的事算什么，只要模模胡胡。模模胡胡的过了新年，仍旧教我的‘子曰诗云’去。” （20）“你教的是‘子曰诗云’”么？我觉得奇异，便问。 （21）“自然。你还以为教的是ABCD么？我先是两个学生，一个读《诗经》，一个读《孟子》。新近又添了一个，女的，读《女儿经》。连算学也不教，不是我不教，他们不要教。” （22）“我实在料不到你倒去教这类书，……” （23）“他们的老子要他们读这些；我是别人，无乎不可的。这些无聊的事算什么？只要随随便便，……” （24）“那么，你以后豫备怎么办呢？” （25）“以后？——我不知道。你看我们那时豫想的事可有一件如意？我现在什么也不知道，连明天怎样也不知道，连后一分……” （26）堂倌送上账来，交给我；他也不像初时候的谦虚了，指向我看一眼，便吸烟听凭我付了账。（27）我们一同走出店门，他所住的旅馆和我的方向正相反，就在门口分别了。我独自向着自己的旅馆走，寒风和雪片扑在脸上，倒觉得很爽快。见天色已是黄昏，和屋宇和街道都织在密雪的纯白而不定的罗网里。1924年2月16日
        \end{CJK} &
        \\
         \hline
        Q1 \begin{CJK}{UTF8}{gbsn}
        下列对文章思想内容的理解与分析，不正确的一项是
        \end{CJK}
         & \\
        A. \begin{CJK}{UTF8}{gbsn}
        “行动却变得格外迂缓，很不像当年敏捷精悍的吕纬甫了”高度概括了眼前吕纬甫的精神状态，突出他的迂缓颓废。
        \end{CJK} & \\
        B. \begin{CJK}{UTF8}{gbsn}
        “蝇子飞了一个小圈子，便又回来停在原地点”，吕纬甫的这番自述自嘲中对自身缺乏清醒的认识，浑噩度日，揭示了残酷的现实生活将人的灵魂挤扁，只能在颓唐消沉中磨蚀生命的主题。$\star$
        \end{CJK} & \\
        C. \begin{CJK}{UTF8}{gbsn}
        从吕纬甫叙述现在教书生涯的内容和原因的话语中，可见他已经违背了当初的理想，变得苟且偷安，屈从于当前顽固封建势力。
        \end{CJK} & \\
        D. \begin{CJK}{UTF8}{gbsn}
        文章通过吕纬甫的人生经历来告诉读者，吕纬甫的人生悲剧正是那个时代无数知识分子悲剧命运的代表，而个人的悲剧背后则是整个时代的悲哀。 
        \end{CJK} & \\
        \\
        Q2 \begin{CJK}{UTF8}{gbsn}
        下列对文章艺术特点的理解与鉴赏，不正确的一项是
        \end{CJK}
         & \\
        A. \begin{CJK}{UTF8}{gbsn}
        小说情节围绕吕纬甫的自述展开，他的叙述中有乡情，有友情，还有“迁坟”这件小事中流露出的人情 $\star$
        \end{CJK} & \\
        B. \begin{CJK}{UTF8}{gbsn}
        梅花、山茶与白雪共同构成了一幅充满生机与活力的画面，表现了鲁迅先生悲观中奋起、绝望中反抗的战斗精神。
        \end{CJK} & \\
        C. \begin{CJK}{UTF8}{gbsn}
        小说人物刻画体现出鲁迅先生简练传神的特色，极具个性化的人物语言，偶一闪现的肖像描写，颇耐人寻味。其中一句“也还是乱蓬蓬的须发”可让人生发许多联想。
        \end{CJK} & \\
        D. \begin{CJK}{UTF8}{gbsn}
        小说结尾含蓄深刻，意蕴无穷。“见天色已是黄昏，和屋宇和街道都织在密雪的纯白而不定的罗网里。” “罗网”是指封建文化思想依旧弥漫的社会环境。
        \end{CJK} & \\
        \\
    \hline
    \end{tabular}
    \caption{A example of Modern Chinese documents along with questions (left) and English translation (right), $\star$ is the correct option.}
    \label{tab:modern_chinese}
\end{table*}

==> 40_approach.tex <==
\section{Approach}
We use Chinese pre-trained BERT as the baseline. In this section, we will introduce BERT and itsand the t for this dataset.
\subsection{BERT}
\label{BERT}
The full name of BERT is Bidirectional Encoder Representation from Transformers, which is a pre-trained language model using Transformers encoder as the core. It is no longer like the previous language model for one-way language model training or shallow splicing of language models in two directions. It builds two pre-training tasks, Masked Language Model (MLM) and Next Sentence Prediction (NSP), which can be used in Semi-supervised learning is performed in a large number of unlabeled corpora, which can generate language representations with contextual information. In the representation of the input sequence, BERT adds [CLS] at the top of each sequence, and adds [SEP] at the end of the first sentence and the latter sentence. At the same time, in order to integrate the semantics, position, and upper and lower sentences of the token, Each token is mapped to token embedding, position embedding, and segmentation embedding, and the sum of the three embeddings is used as the input vector of the model. In downstream tasks, you only need to modify the output layer of the pre-trained BERT and fine-tune the model to achieve good results. Since the launch of BERT, BERT and its improved models have swept the lists of major NLPs.

\subsection{Improved model of BERT}
\label{BERT_family}
In the improved BERT model, RoBERTa removed the NSP in BERT and performed a series of parameter optimizations. ERNIE optimized the BERT mask mechanism to perform entity-level and phrase-level masks. Cui and others of Harbin Institute of Technology IFLYTEK introduced whole word masking (wwm) into the MLM task of BERT. First, the article was divided into word sequences with a Chinese word segmentation tool, and then the whole word was masked. In addition, the team also used more and larger corpus for pre-training, which proved to be effective in many downstream tasks. Later, Cui and others proposed MacBERT, replaced NSP with the Sentence Order Prediction (SOP) task in Albert, and made the following modifications to MLM: 1) wwm and n-gram mask were used. For the n-gram mask strategy, from The ratio of unigram to 4-gram is 40\%, 30\%, 20\%, 10\%, 2) In order to solve the problem that the [MASK] token used by the pre-training MLM will not appear in the fine-tuning stage, they will [MASK] token Replace with words with similar meanings to the original words. The choice of synonyms is based on Word2Vec. If no similar words are found, replace them with random words.
\subsection{Input and output processing}
\label{input_output}
The baseline model of this article is also based on pre-trained BERT, and the following modifications are made to the input layer and output layer. 
The input of this task consists of three parts, which are articles, questions, and options. There are 2-4 options. To enable batch processing, we fill the questions of 2 and 3 options into 4 options. For the convenience of presentation, the following notation is introduced below, the document is denoted as D, the question is denoted as Q, and the answer options are denoted as A1,A2,A3,A4. For the i-th option, we construct an input sequence of [CLS] D [SEP] Q [SEP] Ai [SEP], where D is Segment 1 input by BERT, and Q and Ai are combined as Segment 2. It can be seen from Table ~\ref{tab:statistics} that quite a lot of text length exceeds 512, the maximum length limit of BERT, so we adopt a strategy of intercepting the input sequence. First, we keep the parts of Q and A intact. For D, we assume that the beginning and end of the article usually convey more important information, so we cut off the middle part of D so that the total length of the sequence is maintained at 512.
We selected several commonly used Chinese pre-trained model as the baseline, including Google's BERT-chinese, BERT-multilingual, Baidu's ERNIE, HFL's BERT-wwm, BERT-wwm-ext, and MacBERT. These 6 pre-training models have the same model structure, all of which are 12-layer of Transformer Encoder. Each layer has 12 attention heads and the hidden state is 768. We also applied two large models, Roberta-large and MacBERT-large, both of which have 24 layers and 16 attention heads.
However, due to the different training data, data volume, and pre-training methods used by these pre-training BERTs, the training results are also different. In section ~\label{input_output}, we will compare the results of the 8 baseline models.
BERT will generate a 768-dimensional hidden state for each token of the input sequence. We take the output state of [CLS] token in the 12th layer and map it to a one-dimensional logit through a single-layer neural network. The logit means to what extent Ai is the correct option. In the same way, we can get the logit of the other 3 options, and the probability of the 4 options can be obtained by transforming the 4 logit by softmax. The goal of training is to minimize the four-class cross-entropy between the label probability and the ground truth. In the inferring stage, we just selects the option with the highest probability as the prediction result.
